Tayler-Spruit dynamo in stably stratified rotating fluids: Application to proto-magnetars

The formation of highly magnetized young neutron stars, called magnetars, is still a strongly debated question. A promising scenario invokes the amplification of the magnetic field by the Tayler-Spruit dynamo in a proto-neutron star (PNS) spun up by fallback. Barr\`ere et al. 2023 supports this scenario by demonstrating that this dynamo can generate magnetar-like magnetic fields in stably stratified Boussinesq models of a PNS interior. To further investigate the Tayler-Spruit dynamo, we perform 3D-MHD numerical simulations with the MagIC code varying the ratio between the Brunt-V\"ais\"al\"a frequency and the rotation rate. We first demonstrate that a self-sustained dynamo process can be maintained for a Brunt-V\"ais\"al\"a frequency about 4 times higher than the angular rotation frequency. The generated magnetic fields and angular momentum transport follow the analytical scaling laws of Fuller et al. 2019, which confirms our previous results. We also report for the first time the existence of an intermittent Tayler-Spruit dynamo. For a typical PNS Brunt-V\"ais\"al\"a frequency of $10^{3}\,{\rm s}^{-1}$, the axisymmetric toroidal and dipolar magnetic fields range between $1.2\times 10^{15}-2\times 10^{16}\,{\rm G}$ and $1.4\times 10^{13}-3\times 10^{15}\,{\rm G}$, for rotation periods of $1-10\,{\rm ms}$. Thus, our results provide numerical evidence that our scenario can explain the formation of magnetars. As the Tayler-Spruit dynamo is often invoked for the angular momentum transport in stellar radiative zones, our results are also of particular importance in this field and we provide a calibration of the Fuller et al.'s prescription based on our simulations, with a dimensionless normalisation factor of the order of $10^{-2}$.

==> tabular_output.tex <==
%%
%% Monday 25-03-2024, 20:59:00
%% File generated by table.py
%%
\begin{tabular}{lcccccccccccccr}
\toprule
 Name & ${q}$ & $\Lambda$ & $B_{\mathrm{tor}}^{m=0}$ & $B_{\mathrm{pol}}^{m=0}$ & $B_{\mathrm{dip}}$ & $B_{\mathrm{tot}}^{m\neq 0}$ & $v_{\mathrm{tot}}^{m\neq 0}$ & $B_sB_{\phi}/4\pi$ & $B_s^{m=0}B_{\phi}^{m=0}/4\pi$ & $v_r^{m\neq 0}v_{\phi}^{m\neq 0}/4\pi$ & $v_r^{m\neq 0}v_{\phi}^{m\neq 0}/4\pi$ & $l_{\mathrm{TI}}$ & $P_{\mathrm{cyc}}$ & $\alpha_{\mathrm{cyc}}$ \\
   &   &   & $[10^{14}\,{\rm G}]$ & $[10^{14}\,{\rm G}]$ & $[10^{14}\,{\rm G}]$ & $[10^{14}\,{\rm G}]$ & $[10^7\,{\rm cm}\cdot{\rm s}^{-2}]$ & $[10^{27}\,{\rm G}^2]$ & $[10^{27}\,{\rm G}^2]$ & $[10^{25}\,{\rm cm}^2{\rm s}^{-2}]$ & $[10^{25}\,{\rm cm}^2{\rm s}^{-2}]$ & [km] & [s$^{-1}]$ &   \\
\hline
$ \text{Ro0.75s} $ & $0.06$ & $51.85$ & $8.08$ & $0.68$ & $0.48$ & $3.64$ & $0.20$ & $22.57$ & $4.43$ & $6.31$ & $9.19$ & $2.8$ & -- & -- \\
$ \text{Pm1Pr0.1NO0.25} $ & $0.17$ & $69.03$ & $9.57$ & $0.71$ & $0.54$ & $3.80$ & $0.20$ & $13.86$ & $3.63$ & $6.81$ & $10.81$ & $2.5$ & -- & -- \\
$ \text{Pm1Pr0.1NO0.5} $ & $0.35$ & $74.71$ & $10.33$ & $0.80$ & $0.34$ & $2.59$ & $0.20$ & $8.71$ & $2.79$ & $7.00$ & $12.96$ & $1.5$ & -- & -- \\
$ \text{Pm1Pr0.1NO1} $ & $0.69$ & $99.44$ & $12.12$ & $0.25$ & $0.14$ & $1.02$ & $0.11$ & $4.57$ & $1.29$ & $2.13$ & $4.23$ & $0.8$ & -- & -- \\
$ \text{Pm2Pr0.1NO2} $ & $2.37$ & $251.25$ & $13.89$ & $0.32$ & $0.12$ & $0.43$ & $0.03$ & $3.33$ & $2.53$ & $0.33$ & $1.27$ & $0.6$ & $27$ & $0.66$ \\
$ \text{Pm2Pr0.1NO4} $ & $2.57$ & $332.08$ & $15.88$ & $0.19$ & $0.07$ & $0.24$ & $0.02$ & $2.28$ & $2.13$ & $0.08$ & $0.54$ & $0.4$ & $12$ & $0.59$ \\
$ \text{Pm2Pr0.1NO8} $ & $2.54$ & $531.21$ & $20.25$ & $0.07$ & $0.04$ & $0.23$ & $0.02$ & $2.63$ & $1.57$ & $0.06$ & $0.65$ & $0.2$ & $13$ & $0.38$ \\
$ \text{Pm4Pr0.1NO4} $ & $2.57$ & $478.89$ & $13.56$ & $0.18$ & $0.03$ & $0.14$ & $0.01$ & $0.68$ & $0.96$ & $0.02$ & $0.07$ & $0.4$ & $3$ & $0.62$ \\
$ \text{Pm4Pr0.1NO6} $ & $2.59$ & $495.22$ & $13.82$ & $0.12$ & $0.03$ & $0.12$ & $0.01$ & $0.83$ & $1.02$ & $0.02$ & $0.11$ & $0.3$ & $16$ & $0.5$ \\
$ \text{Pm4Pr0.1NO8} $ & $2.54$ & $714.16$ & $16.58$ & $0.12$ & $0.03$ & $0.11$ & $0.01$ & $0.99$ & $1.15$ & $0.01$ & $0.09$ & $0.2$ & $10$ & $0.47$ \\
$ \text{Pm4Pr0.1NO10} $ & $3.74$ & $862.86$ & $18.24$ & $0.06$ & $0.02$ & $0.08$ & $0.01$ & $0.77$ & $0.80$ & $0.01$ & $0.06$ & $0.15$ & $6$ & $0.57$ \\
\bottomrule
\end{tabular}

